Galclaim: A tool to identify host galaxy of astrophysical transient sources

The Galclaim software is designed to identify association between astrophysical transient sources and host galaxy by computing the probability of chance alignment. It is distributed as an open source Python software. It is already used to identify, confirm or reject host galaxy candidates of GRBs and to validate or invalidate transient candidates in astrophysical observations. Such tools are also very useful to characterise archived transient candidates in large sky survey telescopes.

==> bib.tex <==
@ARTICLE{Leibler10,
       author = {{Leibler}, C.~N. and {Berger}, E.},
        title = "{The Stellar Ages and Masses of Short Gamma-ray Burst Host Galaxies: Investigating the Progenitor Delay Time Distribution and the Role of Mass and Star Formation in the Short Gamma-ray Burst Rate}",
      journal = {\apj},
     keywords = {gamma-ray burst: general, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2010,
        month = dec,
       volume = {725},
       number = {1},
        pages = {1202-1214},
          doi = {10.1088/0004-637X/725/1/1202},
archivePrefix = {arXiv},
       eprint = {1009.1147},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...725.1202L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{         harris2020array,
 title         = {Array programming with {NumPy}},
 author        = {Charles R. Harris and K. Jarrod Millman and St{\'{e}}fan J.
                 van der Walt and Ralf Gommers and Pauli Virtanen and David
                 Cournapeau and Eric Wieser and Julian Taylor and Sebastian
                 Berg and Nathaniel J. Smith and Robert Kern and Matti Picus
                 and Stephan Hoyer and Marten H. van Kerkwijk and Matthew
                 Brett and Allan Haldane and Jaime Fern{\'{a}}ndez del
                 R{\'{i}}o and Mark Wiebe and Pearu Peterson and Pierre
                 G{\'{e}}rard-Marchant and Kevin Sheppard and Tyler Reddy and
                 Warren Weckesser and Hameer Abbasi and Christoph Gohlke and
                 Travis E. Oliphant},
 year          = {2020},
 month         = sep,
 journal       = {Nature},
 volume        = {585},
 number        = {7825},
 pages         = {357--362},
 doi           = {10.1038/s41586-020-2649-2},
 publisher     = {Springer Science and Business Media {LLC}},
 url           = {https://doi.org/10.1038/s41586-020-2649-2}
}
